HomDroid: Detecting Android Covert Malware by Social-Network Homophily Analysis

Android has become the most popular mobile operating system. Correspondingly, an increasing number of Android malware has been developed and spread to steal users' private information. There exists one type of malware whose benign behaviors are developed to camouflage malicious behaviors. The malicious component occupies a small part of the entire code of the application (app for short), and the malicious part is strongly coupled with the benign part. In this case, the malware may cause false negatives when malware detectors extract features from the entire apps to conduct classification because the malicious features of these apps may be hidden among benign features. Moreover, some previous work aims to divide the entire app into several parts to discover the malicious part. However, the premise of these methods to commence app partition is that the connections between the normal part and the malicious part are weak. In this paper, we call this type of malware as Android covert malware and generate the first dataset of covert malware. To detect them, we first conduct static analysis to extract the call graphs. Through the deep analysis on graphs, we observe that although the correlations between the normal part and the malicious part in these graphs are high, the degree of these correlations has a distribution. Based on the observation, we design HomDroid to detect covert malware by analyzing the homophily of call graphs. We identify the ideal threshold of correlation to distinguish the normal part and the malicious part based on the evaluation results on a dataset of 4,840 benign apps and 3,385 covert malicious apps. According to our evaluation results, HomDroid is capable of detecting 96.8% of covert malware while the False Negative Rates of another four state-of-the-art systems (i.e., PerDroid, Drebin, MaMaDroid, and IntDroid) are 30.7%, 16.3%, 15.2%, and 10.4%, respectively.

==> outline/relatedwork.tex <==
\section{Related Work}

\par The Android platform has become the main target of choice for attackers, posing a serious threat to users' safety and privacy. 
Therefore, it is of great significance to establish a healthy mobile app market.
In recent years, academia and industry have done a lot of important studies for completing the purpose.

 \textbf{\emph{1) Syntax-based Android Malware Detection}}
Syntax-based methods \cite{peng2012using, aafer2013droidapiminer, wang2014exploring, arp2014drebin, sarma2012android, zhou2012hey} ignore the semantics of app code to achieve efficient Android malware detection.
For example, Wang \emph{et al.} \cite{wang2014exploring} detects Android malware by analyzing risky permissions requested by an app. 
It scans the manifest file to collect the list of all permissions, and then apply several feature ranking methods to rank them with respect to the risk. 
After obtaining the ranking of all analyzed permissions, permissions with top risks will be considered as risky permissions and are used as features to detect malware.
These risky permissions can provide a mechanism of access control to core facilities of the mobile system, so they can be represented as a type of apps' behavior.
Because of the lack of program semantics, such approach suffers from low effectiveness on detecting Android malware.
\emph{Drebin} \cite{arp2014drebin} considers extracting eight different types of feature sets from an app, four of which are extracted from the manifest file, and the others are obtained from app code. Feature sets in the manifest consists of hardware features, requested permissions, app components, and filtered intents while includes restricted API calls, used permissions, suspicious API calls, and network addresses in app disassembled code. 
After extracting all the feature sets from an app, \emph{Drebin} embeds them into a joint vector space to train an SVM to detect malware.
However, it only searches for the presence of particular strings, such as some restricted API calls, rather than considers the program semantics. So it can be easily evaded by attacks on syntax features \cite{chen2018android}.

 \textbf{\emph{2) Semantics-based Android Malware Detection}}
In order to maintain high effectiveness on detecting Android malware, researchers \cite{zhang2014semantics, feng2014apposcopy, mariconti2016mamadroid, yang2015appcontext, allen2018improving, yang2018enmobile, avdiienko2015mining, machiry2018using} conduct program analysis to extract different types of app semantics.
For example, \emph{MaMaDroid} \cite{mariconti2016mamadroid} first performs static analysis to obtain the graph representation of an app, then all the sequences are obtained from the graph and are abstracted into the corresponding packages to model the app's invocation behaviors. 
It builds a Markov chain model to represent the transition probabilities between functions. 
Markov chains stand for multiple pairs of call relationships performed by an app and are used to construct feature vectors to detect malware.
In practice, the abstraction of \emph{MaMaDroid} may bring some false alarms, for instance, \emph{android.telephony.TelephonyManager.getDeviceId()} and \emph{android.telephony.SmsManager.sendTextMessage()} are both abstracted in \emph{android.telephony} package while their usages and corresponding security-levels are completely different.
The main ideas of \emph{DroidSIFT} \cite{zhang2014semantics} and \emph{Apposcopy} \cite{feng2014apposcopy} are similar, that is, they both first extract graph representation of an app, and then conduct graph matching to detect malware.
However, since heavy-weight program analysis are both performed by \emph{DroidSIFT} and \emph{Apposcopy} to obtain accurate graph, they all suffer from low scalability.
In their papers \cite{zhang2014semantics, feng2014apposcopy}, they report that the average runtime overhead are 175.8 seconds and 275 seconds for \emph{DroidSIFT} and \emph{Apposcopy}, respectively. 
 

\textbf{\emph{3) Repackaged Android Malware Detection}} 
Some approaches \cite{repack1, repack2, repack3, repack4, repack5} aim to detect repackaged Android malware, for example, \emph{MassVet} \cite{repack4} builds a viewgraph to describe an app with a reasonably complicated UI structure. 
To ensure the high scalability on graph matching, \emph{MassVet} applies a similarity comparison algorithm that appeared in their former work \cite{chen2014achieving} to the analysis of the recovered view graph. 
It has validated the high efficiency and scalability of mobile malware detection, however, the original purpose of \emph{MassVet} is to detect repackaged malware. 
It can cause a false negative when the app is a new malware.
\emph{DR-Droid} \cite{repack2} divides the entire app code into multiple dependency-based regions to detect repackaged malware.
The way they partition the app is to generate a class-level dependency graph by exploring different categories of dependencies.
After obtaining the partitioned regions, \emph{DR-Droid} extracts features from each region independently and label it as either benign or malicious.
As long as any region is detected as malicious, the entire app will be considered as a repackaged malware.
The premise of \emph{DR-Droid} to conduct app partition is that the connections between the normal part and the malicious part are weak.
Therefore, when detecting covert malware, it may cause false negatives since the normal part and malicious part are highly correlated.

